Distributionally Robust Statistical Verification with Imprecise Neural Networks

A particularly challenging problem in AI safety is providing guarantees on the behavior of high-dimensional autonomous systems. Verification approaches centered around reachability analysis fail to scale, and purely statistical approaches are constrained by the distributional assumptions about the sampling process. Instead, we pose a distributionally robust version of the statistical verification problem for black-box systems, where our performance guarantees hold over a large family of distributions. This paper proposes a novel approach based on uncertainty quantification using concepts from imprecise probabilities. A central piece of our approach is an ensemble technique called Imprecise Neural Networks, which provides the uncertainty quantification. Additionally, we solve the allied problem of exploring the input set using active learning. The active learning uses an exhaustive neural-network verification tool Sherlock to collect samples. An evaluation on multiple physical simulators in the openAI gym Mujoco environments with reinforcement-learned controllers demonstrates that our approach can provide useful and scalable guarantees for high-dimensional systems.

==> questions_for_michele.tex <==
\section{Questions for Michele}

Note: In our problem setup, we want our family of distributions to only change the distribution of the inputs x. So we should have that $|\mathcal{P}_{Y|X}|=1$ (i.e. the families of distributions only come from $\mathcal{P}_{\mathcal{X}}$).

1) In the proof of theorem 1, we assume that the loss function is optimized (at a local minimum wrt the upper probability function). That means it is optimized wrt all $P_{\mathcal{X}} \in \mathcal{P}_{\mathcal{X}}$, correct? So if we take some other $P'_{\mathcal{X}} \notin \mathcal{P}_{\mathcal{X}}$, will theorem 1 guarantee that: $$\int_\mathcal{X} \underline{P}_{Y\mid X}\left(\{\underline{\Phi}(x)-\lambda\beta \leq y \leq \overline{\Phi}(x)+\lambda\beta\}\right) P'_X(\text{d}x) \geq 1-\frac{1}{\lambda}$$\MRC{my guess is no} {\color{blue} MGC: No; the distribution drift has to happen within the set of distributions. (I'm assuming here you're referring to a possible distribution drift \textit{outside the set} of interest). Typically, objectivist imprecise probabilists are not too concerned with this because if the agent is concerned that a big drift may happen, they prescribe them to specify a larger set.}

\textcolor{red}{SD : In our setting, we are considering minimizing the loss $\mathcal{L}$ w.r.t to some particular distribution $P_\mathcal{X}^i \in \mathcal{P}_\mathcal{X}$. So if we pick another distribution $P_\mathcal{X}^j \in \mathcal{P}_\mathcal{X}$, the guarantee of Theorem 1 still holds. Since, $\mathcal{X}$ is the initial set described in the problem ($X_0$). } {\color{blue}<- exactly}

% {\color{blue} IR: a quick follow-up on this: where can I find the formalization of the argument `` minimize the loss of $P_{X}$ and you assume it is minimized over \mathcal{P}_\mathcal{X}$'' (if it exists)?}

2) Is there a way to sample a family of distributions (e.g., to obtain a training set from it)? \IR{My guess is no, gotta pick a single distribution or impose a meta/compound distribution of distributions} {\color{blue} MGC: I'm not sure I understand this question. Let me try my best with an answer. Using credal sets allows to ``adopt a nonparametric approach retaining the parametric interpretation''. With this I mean the following. You have a set of distributions that play the role of a process (eg a Gaussian process). But instead of losing interpretability as a consequence of using second-order distributions, you retain the interpretation coming from ``regular'' probabilities. In turn, you don't sample distributions (or a family of distributions), but instead the $x$'s and the $y$'s according to the probabilities in $\mathcal{P}_\mathcal{X}$ and $\mathcal{P}_{\mathcal{Y} \mid \mathcal{X}}$. Is this what you meant?}\\
\textcolor{red}{IR: Ok, so how do we sample $x$ from family $\mathcal{P}_\mathcal{X}$?} {\color{blue} MGC: you sample $x$ from $P_{X}$, and you assume $P_{X} \in \mathcal{P}_\mathcal{X}$.}

3) Suppose someone specified two ball-shaped (for some distance metric) families of distributions centered around the uniform distribution. One family has a bigger radius than the other. How will the application of the proposed approach differ for these two families --- at what point(s) will the difference in their radii get picked up? {\color{blue} In this case we have the following. Let $B_{big}$ be the larger ball, and $B_{small}$ be the smaller one. We have that $B_{big} \supset B_{small}$. Now, this implies that $\underline{B}_{big} \leq \underline{B}_{small} \leq \overline{B}_{small} \leq \overline{B}_{big}$, where I used the usual upper and lower bars for upper and lower prob's, respectively. These two sets give rise to two different losses (look how the loss is defined in \ref{loss_funct}). The guarantees we found only hold for the ``right loss'' used for the ``right set of prob's''. In other words, if we minimize the loss function based on $B_{small}$, but then ``use'' a distribution in $B_{big}$, our results may not hold any more. Does this answer the question? }

\textcolor{red}{SD : I am not sure if this question is relevant in our case, since we don't change the size of our initial set, or the $\mathcal{X}$ set if you will.}

\textcolor{blue}{IR: That's fine, thanks. It was a sanity check. }




4) Is that an equivalent statement to Theorem 1?

\begin{theorem}\label{main_thm_MRC}
    Assume that $\mathcal{L}(\underline{\Phi},\overline{\Phi})$ is optimized (i.e. ${\partial \mathcal{L}(\underline{\Phi},\overline{\Phi})}/{\partial \overline{\Phi}(x)}=0$, see \eqref{eq12} for the definition of the partial derivative). Pick any $\lambda>0$ and any pair $(x,y)$ sampled from a distribution in $\mathcal{P}$. Let  $A=\{\underline{\Phi}(x)-\lambda\beta \leq y \leq \overline{\Phi}(x)+\lambda\beta\}$. If $\mathcal{P}_\mathcal{X}$ and $\mathcal{P}_{\mathcal{Y}\mid \mathcal{X}}$ are compact, then\footnote{Here and in the rest of the paper, compact has to be understood with respect to the topologies $\sigma(\text{ba}(\mathcal{A}_\mathcal{X});B(\mathcal{A}_\mathcal{X}))$ and $\sigma(\text{ba}(\mathcal{A}_\mathcal{Y});B(\mathcal{A}_\mathcal{Y}))$, respectively. Recall that  $\text{ba}(\Sigma)$ is the set of all bounded finitely additive (signed) measures on a generic sigma-algebra $\Sigma$, and $B(\Sigma)$ is the set of all bounded and $\Sigma$-measurable functions.} 
    %weak topology.} , for a generic sigma-algebra $\Sigma$.
    $$\underline{\mathbb{E}}_X\left[ \underline{P}_{Y\mid X}(A) \right]=\inf_{P_X\in\mathcal{P}_\mathcal{X}} \int_\mathcal{X} \underline{P}_{Y\mid X}\left(\{\underline{\Phi}(x)-\lambda\beta \leq y \leq \overline{\Phi}(x)+\lambda\beta\}\right) P_X(\text{d}x) \geq 1-\frac{1}{\lambda}.$$
\end{theorem}

If so, note that \eqref{eq12} has a $\sup_{P_{\mathcal{X}}\in \mathcal{P}_{\mathcal{X}}}$ component. So that means we are making an assumption about how the INN behaves over the entire family $\mathcal{P}_{\mathcal{X}}$. Doesn't that mean we would need to train the INN over the entire family $\mathcal{P}_{\mathcal{X}}$ for the theorem to hold (modulo training errors)? {\color{blue} MGC: There is no difference between this and Theorem 1. I don't know if I understood the question well enough, but let me attempt to answer. You train to get $\overline{\Phi}$ and $\underline{\Phi}$. The probabilities in $\mathcal{P}$ are fixed. What you can argue, from an applied point of view, is to minimize the loss with respect to some regular probabilities $P^\star_X$ and $P^\star_{Y\mid X}$ and then, because the sets are assumed compact, you assume that $P^\star_X=\overline{P}_X$ and that $P^\star_{Y\mid X}=\overline{P}_{Y\mid X}$. This way of proceeding has a \textit{core} flavore to it. Does that answer the question?}

\textcolor{red}{MRC: But don't we need to know the correct $P_{X}^*$ and $P_{Y|X}^*$ ahead of time so we can train on them? If not, how do we ensure we picked the correct distributions to train on? What if we pick a really 'easy' distribution $P_{X}^*$ or $P_{Y|X}^*$? Would that result in a different INN than if we had picked a 'hard' $P_{X}^*$ or $P_{Y|X}^*$?}

\textcolor{red}{ SD : So the assumption is that once we pick a training distribution - $P_X^*$, we assume that Theorem $1$ is applicable to all cases where - $ \forall x, P_X (x) < P_X^* (x) = \overline{P}_X (x)$? } 

{\color{blue} MGC: yes exactly, but $P_X^\star$ must be padded. Yesterday I didn't specify this because I was in a rush, but let me be more specific. You should specify a regular $\tilde{P}_X$ and then $P^\star_X = \tilde{P}_X+\epsilon$, for some $\epsilon>0$. This is called $\epsilon$-padding. It means that $P^\star_X(x)=\tilde{P}_X(x)+\epsilon$, for all $x$. You use this $\epsilon$-padded ``distribution'' as a training ``distribution'', and assume that $P_X (x) < P_X^\star (x) = \overline{P}_X (x)$, for all $x$ and all $P_X\in\mathcal{P}_\mathcal{X}$. Is this clear? Same for $P^\star_{X \mid Y}$.}

\textcolor{red}{MRC: But don't we need to validate that assumption somehow?} {\color{blue} MGC: this is something that I'm often times asked by people who don't work with imprecise probabilities. You're making a less stringent assumption than usual. Instead of choosing a distribution and assume that's the correct data generating process, you say "any distribution that is dominated by $P^\star_X$ (or $P^\star_{X \mid Y}$) could be correct one". It's a very general assumption. I don't know how you could validate it, so I don't have an exact answer. Choosing the set comes from similar previous experiments or from subjective beliefs, and you assume the correct distribution is within the set.} \\
 
5) Okay so now this is an important piece of the puzzle. Assume we have a training \textbf{set} $S = \{ (x_i, y_i)_{i=1}^{N} \}$, which was used to train the INN $\{\overline{\Phi}, \underline{\Phi}\}$. How do we define the upper probability $\overline{P}_X$ using this above set ? \\
(I know part of it got answered in the previous questions, but I think a clear step-by-step agreement is needed on this.)

{\color{blue} MGC: I think the misunderstanding here comes from having worked previously with IBNNs. Here the sets $\mathcal{P}_\mathcal{X}$ and $\mathcal{P}_{\mathcal{Y}\mid\mathcal{X}}$ do not depend on the data. I'll give an example of what I mean. We can posit that the $x$'s come from a $1$-dimensional normal $\mathcal{N}(\mu,\sigma^2)$, and let $\overline{P}_X$ be such that its pdf is given by
$$\overline{p}(x)= \frac{1}{\sigma\sqrt{2\pi}} \exp\left(-\frac{(x-\mu)^2}{2\sigma^2}\right) + \epsilon,$$
for all $x$ and for some $\epsilon>0$. As you can see, $\overline{P}_X$ does not depend on the data. Then, you do something similar for $\overline{P}_{Y\mid X}$. Once you have both, the loss becomes 
\begin{align*}
\begin{split}
    {\mathcal{L}}(\underline{\Phi},\overline{\Phi})=  \int_{\mathcal{X}} \bigg[ &\int_{\mathcal{Y}} \max\left(y-\overline{\Phi}(x),0\right)^2 \overline{p}_{Y\mid X}(y)\text{d}y\\
     + &\int_{\mathcal{Y}} \max\left(\underline{\Phi}(x)-y,0\right)^2 \overline{p}_{Y\mid X}(y)\text{d}y + \beta\left( \overline{\Phi}(x)-\underline{\Phi}(x) \right) \bigg] \overline{p}_X(x) \text{d}x.
\end{split}
\end{align*}
Here we're implicitly assuming that the upper probabilities are $2$-alternating, but that's fine. Does this answer the question? The fact that the sets of probabilities and the data points are separated are crucial, especially in light of the difference between network and epistemic uncertainty. Just to be clear: this doesn't mean that you \textit{cannot} make the probability depend on the data, but that you \textit{don't have to}. So, for example, if $\mathcal{X}=[0,5]$ and you observe $x_1=2$, $x_2=3$, and $x_3=1$, you can let $\overline{p}(x_1)=\overline{p}(x_2)=\overline{p}(x_1)=1/3 + \epsilon$ and $\overline{p}(x)= \epsilon$ for all $x\in\mathcal{X}\setminus\{2,3,1\}$, but you don't have to. You could, for example, consider a truncated Normal on $[0,5]$ and $\epsilon$-pad it to obtain the upper probability.} 


\textcolor{red}{SD : Okay, that makes sense. This is good news. For our case then this would simply be a union over intervals in the input space (This is an implementation detail). Another possibly trivial question, how do we choose this $\epsilon$, and also how do we define all such $P$ which is dominated by $\overline{P}$ ? }

{\color{blue} MGC: So $\epsilon$ can be chosen freely, as long as it is positive. You can pick it as small as you want if needed, e.g. $\epsilon=0.01$. Clearly, the larger $\epsilon$ is, the more distributions are dominated by $\overline{P}$. All the (countably additive) distributions that are dominated by $\overline{P}$ belong to the core of $\overline{P}$, 
\begin{align*}
   \text{core}(\overline{P}):=\{&P \in \Delta(\Omega,\mathcal{F}): P(A) \leq \overline{P}(A), \forall A \in \mathcal{F}\} \nonumber\\ 
   =\{&P \in \Delta(\Omega,\mathcal{F}): \overline{P}(A) \geq P(A) \geq \underline{P}(A) \text{, } \forall A \in \mathcal{F}\},
\end{align*}
that is nonempty by construction -- by the way we specified $\overline{P}$ via the $\epsilon$-padding. It is also convex and compact in the weak$^\star$ topology. That could be our $\mathcal{P}$. But it \textit{doesn't have to be that}; we could also simply specify a finite amount of distributions that are dominated by $\overline{P}$. There is always at least one, because again the core is nonempty. In that case, the set $\mathcal{P}$ would be compact as well (because it's finite), but not convex (we don't need convexity of the set of probabilities, so we're ok with that).}

\textcolor{red}{SD :  I am slightly confused as to why the number of samples wouldn't have an affect on how we define $\overline{P}$. Because somehow the training set $S$ decides the distribution over which $\{\overline{\Phi}, \underline{\Phi} \}$'s was trained. For instance, $S$ could be $10$ samples distributed uniformly in the intervals $[2,4]$ and $[5,9]$, where, $\mathcal{X} = [0,15]$. In that, case what is $\overline{P}$ ?   (I think I would be happier if my suspicion about $S$ dependency is wrong here)}


{\color{blue}MGC: In the non-imprecise case, the probability does not depend on the number of samples either. I don't understand why this is confusing to you. The answer that I'd give is the same as before. Let me give you another example. Consider a simple probability inequality like Markov inequality. In that case, if $X>0$ you say that for all $a>0$, $\mathbb{P}(X \geq a) \leq \mathbb{E}(X)/a$. Probability $\mathbb{P}$ does not depend on the number of samples. Similarly, the imprecise version would look something like $\overline{\mathbb{P}}(X \geq a) \leq \overline{\mathbb{E}}(X)/a$. This because we posit that the true $\mathbb{P}$ lives in $[\underline{\mathbb{P}},\overline{\mathbb{P}}]$. Basically, $\mathbb{P}$ is the true data generating process, which is not affected by the number of samples. Does this make sense?}

==> tab_beta_3_combo.tex <==
\begin{table}[!htb]
    \begin{minipage}{\linewidth}
      \centering
        \input{tab_beta_3}
    \end{minipage}%

    \begin{minipage}{\linewidth}
      \centering
      \input{tab_ood_beta_3}
    \end{minipage} 
    % \caption{Global caption}
\end{table}

% \begin{table}[!htb]
%     \begin{minipage}{.48\linewidth}
%       \centering
%         \input{tab_beta_3}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}{.48\linewidth}
%       \centering
%       \input{tab_ood_beta_3}
%     \end{minipage} 
%     % \caption{Global caption}
% \end{table}

==> water_tank_experiments.tex <==
\subsection{Water Tanks}

\textcolor{red}{MC: I'm putting some of the water tank results here so people can get a feel for how we present the results. }
\begin{itemize}
    \item Put figure of the water tank safety curve
    \item Put figures of a few steps of the active learning
    \item Put figures after the full active learning with and without the inflation and showing the individual NNs of the INNs
    \item Show INN loss over each iteration, both with and without active learning (Need to generate this plot on my end)
\end{itemize}


\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{Figures/waterTank/gtProbs.png}
        \caption{Ground truth safety probabilities for a 1D cross section of the water tank initial states.}
        \label{fig:waterTankGTProbs}
\end{figure}



\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/waterTank/activeLearning/exINNErrorsNoLambdaTrial6.png}
        \caption{INN error after 7 steps of active learning} 
        \label{fig:4stepAhead}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/waterTank/activeLearning/exINNErrorsNoLambdaTrial13.png}
        \caption{INN predictions after 14 steps of active learning} 
        \label{fig:10stepAhead}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/waterTank/activeLearning/exINNErrorsNoLambdaTrial19.png}
        \caption{INN predictions after 20 steps of active learning} 
        \label{fig:15stepAhead}
    \end{subfigure}
    \caption{INN safety predictions (both upper and lower) for a 1D cross section of water tank states.}
    \label{fig:ORCAErrScatter}
\end{figure}


\begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/waterTank/exINNErrors.png}
        \caption{INN predictions without inflation (i.e. with no guarantee)} 
        \label{fig:4stepAhead}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/waterTank/exINNErrorsNoLambda.png}
        \caption{INN predictions with inflation (i.e. with a guarantee)}
        \label{fig:10stepAhead}
    \end{subfigure}
    \caption{INN safety predictions with and without the $\lambda$ and $\beta$ inflation that is necessary for the guarantee.}
    \label{fig:ORCAErrScatter}
\end{figure}


